Pseudorandom Generators for Polynomial Threshold Functions

We study the natural question of constructing pseudorandom generators (PRGs) for low-degree polynomial threshold functions (PTFs). We give a PRG with seed-length log n/eps^{O(d)} fooling degree d PTFs with error at most eps. Previously, no nontrivial constructions were known even for quadratic threshold functions and constant error eps. For the class of degree 1 threshold functions or halfspaces, we construct PRGs with much better dependence on the error parameter eps and obtain a PRG with seed-length O(log n + log^2(1/eps)). Previously, only PRGs with seed length O(log n log^2(1/eps)/eps^2) were known for halfspaces. We also obtain PRGs with similar seed lengths for fooling halfspaces over the n-dimensional unit sphere. The main theme of our constructions and analysis is the use of invariance principles to construct pseudorandom generators. We also introduce the notion of monotone read-once branching programs, which is key to improving the dependence on the error rate eps for halfspaces. These techniques may be of independent interest.

==> derandhs.tex <==
\subsection{Derandomizing $G_{reg}$}
We now study derandomize the construction of $G_{reg}$ using Nisan's PRG for space-bounded computations. From Theorem~\ref{mainhs}, $G_{reg}$ fools halfspaces and has seed-length $O(\log n \log^3(1/\epsilon)/\epsilon^2)$. We derandomize $G_{reg}$ to obtain a PRG $G_N$ fooling halfspaces with seed-length $O(\log n \log(1/\epsilon) + \log^{2.5}(1/\epsilon)\log\log(1/\epsilon))$. The derandomization also works with other PRGs for space-bounded computations such as those of Nisan and Zuckerman and Impagliazzo et al.\\

The derandomization is motivated by the fact that for a fixed hash function $h$, and $w \in \rn, \theta \in \reals$, the distribution of $\sgn(\,\iprod{w}{G_{reg}(h,z^1,\ldots,z^t)}-\theta\,)$ can be approximated by a small-space branching program with $t$ layers. Given this observation, instead of choosing $z^1,\ldots,z^t$ independently as before, we can choose them from the output of a PRG small-space computations reducing the randomness used significantly. We in fact show that PRGs for small-space machines fool low-degree {\sl monotone} machines, as defined below, even when the space used is large. We first need some definitions.
\begin{definition}
A $(S,D,T)$-space machine $M$ is a layered multi-graph with a layer for each $1 \leq i \leq T+1$ and at most $2^{S}$ vertices (states) in each layer. The first layer has a single vertex $M_0$ and each vertex in the last layer is labeld with $0$ (rejecting) or $1$ (accepting). For $1 \leq i \leq T$, a vertex $v$ in layer $i$ has at most $2^D$ outgoing edges each labeled with an element of $\{0,1\}^D$ and ending at a vertex in layer $i+1$. 
%The vertices in a layer are labeled $1,\ldots,2^{S}$ and a vertex $v_{ij}$ with label i in layer $j$ has at most $2^D$ outgoing edges to layer $j+1$ each labeled with an element of $\{0,1\}^S$. 
\end{definition}

Let $M$ be a $(S,D,T)$-space machine $M$ and let $v$ be a vertex of $M$ in layer $i$. For $z = (z^{i},z^{i+1},\ldots,z^T) \in (\{0,1\}^D)^{T-i}$ call $(v,z)$ an {\sl accepting} pair if starting from $v$ and taking the path with edges labeled $z$ in $M$ we land at an accepting state. Also, let $A_M(v) = \{z: (v,z) \text{ is accepting in $M$}\}$.

\begin{definition}
A function $G:\{0,1\}^r \rgta (\{0,1\}^S)^T$ is said to fool $(S,D,T)$-space machines with error $\epsilon$ if for all $(S,D,T)$-space machines $M$ the following holds.
\[|\, \pr_{z \in_u (\{0,1\}^S)^T}\,[(M_0,z) \text{ is an accepting pair}] - \pr_{y \in_u \{0,1\}^r}\,[(M_0,G(y)) \text{ is an accepting pair}]\,| \leq \epsilon.\]
\end{definition}

Nisan, Impaglizzo et al.~give PRGs that fool $(S,D,T)$-space machines with error $\exp(2^{-\Omega(S+D)})$ and seed-length $r = O((S+D)\log T)$. Here we work with Nisan's PRG and show that Nisan's PRG in fact fools arbitrary space, low-degree {\sl monotone} space-bounded machines as defined below.

\begin{definition}[Monotone Branching Programs]
A $(S,D,T)$-space machine is said to be monotone if the following holds. For $1 \leq i \leq T$, there exists an ordering $\{v_1,\ldots,v_{L_i}\}$ of the vertices in layer $i$ so that for $1 \leq j < k \leq L_i$, $A_M(v_j) \subseteq A_M(v_k)$. 
\end{definition}

\begin{theorem}\label{monotonebp}
Let $0 < \delta < 1$ and $N:\{0,1\}^R \rgta (\{0,1\}^D)^T$ be Nisan's PRG fooling $(\log(1/\delta T),D,T)$-space machines. Then, $N$ fools monotone $(S,D,T)$-machines for arbitrary $S$ with error at most $\exp(-\Omega(D))+\delta$. 
\end{theorem}

In particular, the above theorem gives a PRG for fooling monotone $(S,D,T)$-space machines with error at most $\exp(-\Omega(D))+\delta$ and seed-length $O(\log(1/\delta)\log T + D \log T)$. We first show how to derandomize $G_{reg}$ assuming the above theorem.\\

Let $s,t,m,K=K(\epsilon)$ be set as in the context of Theorem~\ref{mainhs}. Let $s_0 = K(\epsilon)/\epsilon$ and let $N:\{0,1\}^r \rgta (\{0,1\}^s)^t$ be Nisan's pseudorandom generator fooling $(s_0,s,t)$-space machines with error $\exp(2^{-\Omega(s)})$ and seed-length $r = O((s_0+s) \log t) = O(s \log t)$. Define $G_N: \hh \times \{0,1\}^r \rgta \dpm^n$ by 
\begin{equation}\label{gnisan}
  G_N(h,y) = G_{reg}(h,N(y)).
\end{equation}
We show that $G_N$ fools halfspaces with error at most $O(\epsilon)$ by showing that for a fixed hash function $h,w \in \rn, \theta \in \reals$, $\sgn(\iprod{w}{G_{reg}(h,z)}-\theta)$ can be computed by a monotone low-degree branching program.
\begin{theorem}[Main]\label{derandhs}
$G_N$ fools halfspaces with error $O(\epsilon)$ and seed-length $O(\log n \log(1/\epsilon) + s \log t) =  O(\,\log n \log(1/\epsilon) + \log^{2.5}(1/\epsilon)\log\log(1/\epsilon)\,)$. 
\end{theorem}   
\begin{proof}
Fix a halfspace $\hwt$. Without loss of generality (see \cite{LewisC67} for instance) suppose that $w_i,\theta$ are integers. Let $N = n \max_i (|w_i|,|\theta|)$. Observe that for any $x \in \dpm^n$, $\iprod{w}{x}-\theta \in \{-N,-N+1,\ldots,0,\ldots,N\}$. Fix a hash function $h \in \hh$. We define a $(\log N,s,t)$-space machine $M_{h,w}$ that for $z = (z^1,\ldots,z^t) \in (\{0,1\}^s)^t$ computes $\iprod{w}{G_{reg}(h,z)}$.\\

For $1 \leq i \leq t$, let $w^i = w_{|h^{-1}(i)}$. Then, for $z = (z^1,\ldots,z^t) \in (\{0,1\}^s)^t$,  by definition of $G_{reg}$ Equation \eqref{genreg}, 
\[ \iprod{w}{G_{reg}(h,z^1,\ldots,z^t)} = \sum_{i=1}^t \iprod{w^i}{G_0(z^i)}.\]
Define $M_{h,w}$ as follows. For each $0 \leq i \leq t$, put $N$ nodes in layer $i$ with labels $1,\ldots,N$. The vertices in layer $i$ correspond to the partial sums $Z_i = \sum_{l=1}^i \iprod{w^l}{G_0(z^l)}$.  Note that all partial sums $Z_i$ lie in $\{-N,-N+1,\ldots,N\}$. Now, given the partial sum $Z_i$ there are $2^s$ possible values for $Z_{i+1}$ ranging in $\{Z_i + \iprod{w^{i+1}}{G_0(z)}: z \in \{0,1\}^s\}$. We add $2^s$ edges correspondingly. Finally, label all vertices in the final layer corresponding to numbers less than $\theta$ as rejecting and label all other vertices as accepting states.\\

It follows from the definition of $M_{h,w}$ that for $z = (z^1,\ldots,z^t) \in (\{0,1\}^s)^t$, $M_{h,w}(z)$ is an accepting state if and only if $\sgn(\sum_i\iprod{w^i}{G_0(z^i)}-\theta) = \hwt(G_{reg}(h,z))= 1$. It also follows easily that $M_{h,w}$ is monotone. Thus, from Theorem~\ref{monotonebp}, for a fixed $h \in \hh$,
\[| \pr_{z \in_u (\{0,1\}^s)^t}\,[\hwt(G_{reg}(h,z))= 1] - \pr_{y \in_u \{0,1\}^r}\,[\hwt(G_{reg}(h,N(y)))= 1] | \leq \epsilon .\]

From the above and Theorem~\ref{mainhs} it follows that $G_N$ fools halfspaces with error at most $O(\epsilon)$.$\Box$
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "prgthreshold"
%%% End: 


==> regularptf1.tex <==
\section{Fooling Regular Threshold Functions}
We now extend our result for fooling regular halfspaces, Theorem~\ref{regularhs}, to {\sl regular} polynomial threshold functions. Our analysis is based on the generalized Berry-Esseen type theorems for regular low-degree multi-linear polynomials proved by Mossel et al.~and exploits the fact that most of their arguments work even for distributions with bounded independence.
\begin{definition}
Let $P(u_1,\ldots,u_n) = \sum_{I} \alpha_I \prod_{i \in I} u_i$ be a multi-linear polynomial of degree $d$. We will assume through out that $P$ is normalized with $\|P\|_2^2 = \sum_I \alpha_I^2 \leq 1$. We say $P$ is $\epsilon$-regular if for all $i$,
\[ \tau_i(P) = \sum_{I \ni i} \alpha_I^2 \leq \epsilon^2 .\]
We say a polynomial threshold function $f(x) = \sgn(P(x) - \theta)$ is $\epsilon$-regular if $P$ is $\epsilon$-regular.
\end{definition}

Fix $d > 0$. Let $t = 1/\epsilon^2, m = n/t$ and let $\hh$ be an $\alpha$-almost pairwise independent family as in Theorem~\ref{regularhs}. We assume $G_0:\{0,1\}^s \rgta \dpm^m$ to generate a $4d$-wise independent space, generalizing the assumption of $4$-wise independence used for fooling regular halfspaces. 
\begin{theorem}\label{regularptf}
Let $\hh$ be an $\alpha$-almost pairwise independent family for $\alpha = O(1)$ and let $G_0$ generate a $4d$-wise independent distribution. Then, $G_{reg}$ defined by Equation \eqref{genreg} fools $\epsilon$-regular PTFs of degree at most $d$ with error at most $O(\epsilon^{2/4d+1})$ and seed-length $O(\log n/\epsilon^2)$.
\end{theorem}

Theorem~\ref{regularptfi} stated in the introduction follows directly from the above theorem. We first prove some useful lemmas.
\begin{lemma}\label{influence}
For a multi-linear polynomial $P$ of degree $d$, $\sum_j \tau_j(P) \leq d$.
\end{lemma}
The following lemma generalizes Lemma~\ref{hashing} and says that for pairwise independent hash functions and regular polynomials, the total influence is {\sl almost equidistributed} among the buckets.
\begin{lemma}\label{hashingptf}
Let $\mathcal{H}: [n] \rgta [t]$ be a $\delta$-almost pairwise independent family of hash functions. Let $P$ be a $\epsilon$-regular multi-linear polynomial of degree $d$ with coefficients $(\alpha_J)_{J\subseteq [n]}$ and for $h \in \mathcal{H}$ let
\[ \tau(h,i) = \sum_{J \cap h^{-1}(i) \neq \emptyset} \alpha_J^2.\]
Then, for $h \in_u \mathcal{H}$
\begin{equation}\label{hashing1}
  \ex_{h}\left[\, \sum_{i=1}^t \tau(h,i)^2\,\right] \leq \epsilon^2 d + \frac{(1+\delta)d^2}{t}.
\end{equation}
\end{lemma}
\begin{proof}
Fix a $i \in [t]$ and for $1 \leq j \leq n$, let $X_j$ be the indicator variable that is $1$ if $h(j) = i$ and $0$ otherwise. Now,
\begin{align*}\label{}
  \tau(h,i)= \sum_{J \cap h^{-1}(i) \neq \emptyset} \alpha_J^2 &= \sum_{J} \alpha_J^2\, (\vee_{j \in J} X_j) \\
&\leq \sum_{J} \alpha_J^2 \left( \sum_{j \in J} X_j\right)\\
&= \sum_j X_j \sum_{J: J\ni j} \alpha_J^2 \\
&= \sum_{j} X_j \tau_j.
\end{align*}

Thus,
\[ \tau(h,i)^2 \leq \left(\sum_{j=1}^n X_j \tau_j \right)^2 = \sum_j X_j^2 \tau_j^2 + \sum_{j\neq k} X_j X_k \tau_j \tau_k.\]

Note that $\ex[X_j] = 1/t$ and for $j \neq k$, $\ex[X_j X_k] \leq (1+\delta)/t^2$. Thus, 
\begin{align*}\label{}
\ex[\, \tau(h,i)^2\,] &\leq \frac{1}{t}\sum_j \tau_j^2 + \sum_{j\neq k} \tau_j \tau_k \frac{1+\delta}{t^2}\\
&\leq \frac{1}{t}\sum_j \tau_j^2 + \frac{1+\delta}{t^2} (\sum_j \tau_j)^2 \\
&\leq \frac{1}{t} (\max_j \tau_j ) \sum_j \tau_j + \frac{1+\delta}{t^2} (\sum_j \tau_j)^2\\
&\leq \frac{1}{t} \epsilon^2 d + \frac{1+\delta}{t^2} d^2.
\end{align*}

The lemma follows by using Lemma~\ref{influence} and summing over all $i\in[t]$.$\Box$
\end{proof}
We also need the following structural result of Mossel et al.~that reduces the problem of fooling threshold functions to that of fooling certain {\sl nice} functions which are easier to analyze. 
\begin{definition}
  A function $\psi: \reals \rgta \reals$ is $B$-nice, if $\psi$ is smooth and $|\psi^{''''}(t)| \leq B$ for all $t \in \reals$.
\end{definition}

\begin{lemma}\label{nicetoerr}
Let $X,Y$ be two real-valued random variables. If for all $1$-nice functions $\psi$, $|E[\psi(X)] - E[\psi(Y)]| \leq \epsilon$, then for all $t$, $|\pr[X > t]  - \pr[Y>t]| \leq O(\epsilon^{1/(4d+1)})$.
\end{lemma}

Thus, to show that $G_{reg}$ fools regular PTFs, Theorem~\ref{regularptf}, it is enough to show the following.
\begin{lemma}\label{foolnice}
For all $1$-nice functions $\psi$, and $n$-variate multi-linear polynomials $P$ of degree $d$ with $\|P\|_2 \leq 1$,
\[ |E[\psi(P(\overline{Y}))] - E[\psi(P(\overline{Z}))]| \leq O(\max_i \tau_i(P))\]
where $\overline{Y}$ is the uniform distribution over $\dpm^n$ and $\overline{Z}$ is the output of $G_{reg}$.
\end{lemma}
\begin{proof}
Fix a hash function $h \in \hh$. Let $Z_1,\ldots,Z_t$ be $t$ independent samples generated from the $4d$-wise independent space. Let $Y_1,\ldots,Y_t$ be $t$ independent samples chosen uniformly from $\dpm^m$. We will prove the claim via a hybrid argument where we replace the blocks $Y_1,\ldots,Y_t$ with $Z_1,\ldots,Z_t$ progressively.\\

For $0 \leq i \leq t$, let $X^i$ be the distribution with $X^i_{|h^{-1}(j)} = Z_j$ for $1 \leq j \leq i$ and $X^i_{|h^{-1}(j)} = Y_j$ for $i < j \leq t$. Then, for a fixed hash function $h$, $X^0$ is uniformly distributed over $\dpm^n$ and $X^t$ is distributed as the output of the generator. For $i \in [t]$, let $\tau(h,i)$ be the influence of the $i$'th bucket under $h$, 
\[ \tau(h,i) = \sum_{J \cap h^{-1}(i) \neq \emptyset} \alpha_J^2.\]

\begin{claim}\label{hybridstep}
For $0 \leq i < t$, 
\[ |\ex[\psi(P(X^i))] - \ex[\psi(P(X^{i-1}))]| \leq O(9^d \,\tau(h,i)^2).\]
\end{claim}
\begin{proof}
Let $I = h^{-1}(i)$ be the variables that have been changed from $X^{i-1}$ to $X^{i}$. Without loss of generality suppose that $I = \{1,\ldots,m\}$. Let 
\[ P(u_1,\ldots,u_n) = R(u_{m+1},\ldots,u_n) + \sum_{J: J \cap [m] \neq \emptyset} \alpha_J \,\left(\prod_{j \in J} u_j \right),\]
where $R(\;)$ is a multi-linear polynomial of degree at most $d$. Let $S(u_1,\ldots,u_m,u_{m+1},\ldots,u_n)$ denote the degree $d$ multi-linear polynomial given by the second term in the above expression.\\

Observe that $X^{i-1},X^i$ agree on coordinates not in $[m]$. Let $X^{i} = (Z_{1},\ldots,Z_{m},X_{m+1},\ldots,X_n) = (Z,X)$ and $X^{i-1} = (Y_{1},\ldots,Y_{m},X_{m+1},\ldots,X_n) = (Y,X)$. 
Then, 
\[ P(X^{i}) = R(X) + S(Z,X), \;\;\; P(X^{i-1}) = R(X) + S(Y,X) .\]

Now, by using the Taylor series expansion for $\psi$ at $R(X)$,
\begin{multline*}
  \ex[\psi(P(X^i))] - \ex[\psi(P(X^{i-1}))] = \ex[\psi(R + S(Z,X))] - E[\psi(R + S(Y,X))] \\
=\ex[\,\psi(R) + \psi^{'}(R) S(Z,X) + \frac{\psi^{''}(R)}{2}S(Z,X)^2 + \frac{\psi^{'''}(R)}{6}S(Z,X)^3 + \{\leq \frac{1}{24}S(Z,X)^4\}\,] - \\
 \ex[\,\psi(R) + \psi^{'}(R) S(Y,X) + \frac{\psi^{''}(R)}{2}S(Y,X)^2 + \frac{\psi^{'''}(R)}{6}S(Y,X)^3 + \{\leq \frac{1}{24}S(Y,X)^4\}\,] 
\end{multline*}

Observe that $X,Y,Z$ are independent of one another and are $4d$-wise independent individually. Since $S(\;)$ has degree at most $d$, it follows that for a fixed assignment of the variables $X_{m+1},\ldots,X_n$ in $X$,
\[ \ex[S(Z,X)] = \ex[S(Y,X)],\;\; \ex[S(Z,X)^2] = \ex[S(Y,X)^2],\]
\[ \ex[S(Z,X)^3] = \ex[S(Y,X)^3],\;\; \ex[S(Z,X)^4] = \ex[S(Y,X)^4] .\]
Combining the above equations we get 
\begin{equation}\label{pf1}
|\ex[\psi(P(X^i))] - \ex[\psi(P(X^{i-1}))]| \leq \frac{1}{12} \ex[\, S(Y,X)^4\,] .  
\end{equation}

Now, using the fact that $S(\;)$ is a multi-linear polynomial of degree at most $d$ and since $(Y,X)$ is $4d$-wise independent, $\ex[\,S(Y,X)^4\,] = \ex[\,S(W)^4\,]$, where $W$ is uniformly distributed over $\dpm^n$. Also note that 
\begin{align*}\label{}
  \ex[S(W)^2] &= \ex\left[\, \left(\,\sum_{J: J \cap [m] \neq \emptyset} \alpha_J \,\left(\prod_{j \in J} W_j \right)\,\right)^2\,\right] \\
&=  \sum_{J: J \cap I \neq \emptyset} \alpha_J^2 \\
&= \tau(h,i).
\end{align*}

Therefore, using the $(2,4)$-hypercontractivity inequality $\ex[S(W)^4] \leq 9^d\, \ex[S(W)^2]^2$ and Equation \eqref{pf1},
\begin{align*}\label{}
   |\ex[\psi(P(X^i))] - \ex[\psi(P(X^{i-1}))]| &\leq O(\, \ex[\, S(Y,X)^4\,]\,) = O(\, \ex[\,S(W)^4\,]\,)\\
&\leq O(\, 9^d \, \ex[S(W)^2]^2\,) \\
%&\leq O(1) \;9^d\;\left( \sum_{J: J \cap I \neq \emptyset} \alpha_J^2 \right)^2\\
&= O(\, 9^d\, \tau(h,i)^2\,).\Box
\end{align*}
\end{proof}
\end{proof}
\begin{proof}[Proof of Lemma~\ref{foolnice}]
From Claim~\ref{hybridstep}, for a fixed hash function $h$ we have
\[
|\ex[\psi(P(\overline{Y}))] - \ex[\psi(P(\overline{Z}))]| \leq \sum_{i=1}^t |\ex[\psi(P(X^i))] - \ex[\psi(P(X^{i-1}))]| \leq O(1)\, 9^d \,\sum_{i=1}^t \tau(h,i)^2.
\]

Therefore, for $h \in_u \hh$, using Lemma~\ref{hashing} and $t = 1/\epsilon^2, \delta = O(1)$,
\[ |\ex[\psi(P(\overline{Y}))] - \ex[\psi(P(\overline{Z}))]| \leq  O(1)\, 9^d \,\ex_h\left[\sum_{i} \tau(h,i)^2\right] \leq O(\, \epsilon^2\,).\Box\] 
\end{proof}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "prgthreshold"
%%% End: 

